WHFast512: A symplectic N-body integrator for planetary systems optimized with AVX512 instructions

We describe the implementation of the symplectic N-body integrator WHFast512 using Single Instruction Multiple Data (SIMD) parallelism and 512-bit Advanced Vector Extensions (AVX512). We are able to speed up integrations of planetary systems by up to 4.7x compared to the non-vectorized version of WHFast. WHFast512 can integrate the Solar System with 8 planets for 5 billion years in less than 1.4 days. To our knowledge, this makes WHFast512 the fastest direct N-body integrator for systems of this kind. As an example, we present an ensemble of 40-Gyr integrations of the Solar System. Ignoring the Sun's post-main sequence evolution, we show that the instability rate is well captured by a diffusion model. WHFast512 is freely available within the REBOUND package.

==> mnras_jdf.tex <==
\def \aaps{A\&AS}
\def \aap{A\&A}
\def \ag{Astron.~Geophys.}
\def \grl{Geophy.~Research~Letters}
\def \aj{AJ}
\def \al{Astron.~Lett.}
\def \anp{Ann.~Phys.}
\def \apss{Ap\&SS}
\def \apb{Appl.~Phys.~B}
\def \apjl{ApJ}
\def \apjs{ApJS}
\def \apj{ApJ}
\def \ap{Appl.~Phys.}
\def \araa{ARA\&A}
\def \arns{Annu.~Rev.~Nuc.~Sci.}
\def \ar{Astron.~Rep.}
\def \asp{Astron.~Soc.~Pac.}
\def \baas{BAAS}
\def \baps{Bull.~Am.~Phys.~Soc.}
\def \bist{Bull.~Inf.~Sci.~Tech.}
\def \ca{Comments~on~Astrophys.}
\def \cjp{Canadian~J.~Phys.}
\def \cqg{Classical~Quantum~Gravity}
\def \epjc{Euro.~Phys.~J.~C}
\def \gca{Geochimica~et~Cosmochimica~Acta}
\def \grg{Gen.~Relativ.~Gravitation}
\def \icarus{Icarus}
\def \ijmpd{Int.~J.~Mod.~Phys.~D}
\def \jesrp{J.~Electron~Spectrosc.~Related~Phenomena}
\def \jhep{J.~High~Energy~Phys.}
\def \jms{J.~Molecular~Spectrosc.}
\def \josb{J.~Opt.~Soc.~Am.~B}
\def \jos{J.~Opt.~Soc.~Am.}
\def \jpb{J.~Phys.~B}
\def \jpcrds{J.~Phys.~Chem.~Ref.~Data~Suppl.}
\def \jpcrd{J.~Phys.~Chem.~Ref.~Data}
\def \jqsrt{J.~Quant.~Spectrosc.~Radiat.~Transfer}
\def \jtp{J.~Technical~Phys.}
\def \lp{Laser~Phys.}
\def \lnp{Lecture~Notes~Phys.}
\def \met{Metrologia}
\def \mnras{MNRAS}
\def \mpla{Mod.~Phys.~Lett.~A}
\def \nat{Nat}
\def \na{New~Astron.}
\def \nar{New~Astron.~Rev.}
\def \npa{Nucl.~Phys.~A}
\def \npb{Nucl.~Phys.~B}
\def \nsrds{Natl.~Stand.~Rel.~Data~Ser.}
\def \nw{Naturwiss.}
\def \pasa{Publ.~Astron.~Soc.~Aust.}
\def \pasj{Publ.~Astron.~Soc.~Japan}
\def \pasp{PASP}
\def \pawk{Preuss.~Akad.~Wiss.~K}
\def \planss{Planet. Space Sci.}
\def \plb{Phys.~Lett.~B}
\def \phd{PhD~thesis}
\def \pra{Phys.~Rev.~A}
\def \prb{Phys.~Rev.~B}
\def \prc{Phys.~Rev.~C}
\def \prd{Phys.~Rev.~D}
\def \prl{Phys.~Rev.~Lett.}
\def \prsa{Proc.~R.~Soc.~A}
\def \prep{in~preparation}
\def \pr{Phys.~Rev.}
\def \psc{Phys.~Scr.}
\def \ptp{Progress~Theor.~Phys.}
\def \ptrsla{Phil.~Trans.~R.~Soc.~London}
\def \rmp{Rev.~Mod.~Phys.}
\def \rpp{Rep.~Prog.~Phys.}
\def \spu{Sov.~Phys.~Uspekhi}
\def \ssr{Space~Sci.~Rev.}
\def \tms{Trans.~Math.~Software}
\def \za{Z.~Astrophys.}
\def \zpa{Z.~Phys.~A}
\def \zp{Z.~Phys.}

